Novel approaches in Hadron Spectroscopy

The last two decades have witnessed the discovery of a myriad of new and unexpected hadrons. The future holds more surprises for us, thanks to new-generation experiments. Understanding the signals and determining the properties of the states requires a parallel theoretical effort. To make full use of available and forthcoming data, a careful amplitude modeling is required, together with a sound treatment of the statistical uncertainties, and a systematic survey of the model dependencies. We review the contributions made by the Joint Physics Analysis Center to the field of hadron spectroscopy.

==> sections/prod-general-inclusive.tex <==
\label{S:general_inclusive}
High-energy two-body scattering cross sections are dominated by the production of many-body final states. This leads to difficulties in the analysis of individual produced particles: Experimentally assuring that a particular state has been singled out from the bulk of particles produced becomes cumbersome and most times model-dependent. While these challenges are true for any type of produced particle, they are especially hindering in the case of neutral or unstable final states. At the same time, from the theoretical perspective, the rise in number of particles involved leads to a dramatic increase in the independent variables that need to be dealt with.
%
For these reasons, the study of semi-inclusive processes may offer advantages~\cite{Collins:1977jy}: Except for a small chosen set, there is no need to identify the particles in the final state. One needs only to measure the momentum of the singled out particles, and therefore drastically reduces the number of independent variables. In addition, compared to exclusive processes, the cross sections are larger, therefore being experimentally better achievable.

In general, one can write down the semi-inclusive production of a single detected particle from two-body scattering as $a(p_a) + b (p_b) \to c(p_c) + X$, where $p_i$  are the momenta of the particles $i$ of mass $m_i$. The unobserved particles $X$ have a total invariant mass $M$.  A minimal and sufficient subset of invariants (Mandelstam variables) is then given by
%
\begin{equation}
s = (p_a+p_b)^2, \quad t = (p_a-p_c)^2, \quad M^2  = (p_a+p_b-p_c)^2.
\end{equation}
%
For the purpose of this review, we shall focus on the semi-inclusive photoproduction off proton targets, meaning that $m_a$ and $m_b$ are set to $0$ and the nucleon mass $m$, respectively. Furthermore, the minimal value for $M$ is $M_\text{min}=m$. Ultimately, the goal is to study the photoproduction of quarkonia $\mathcal{Q}$ with mass $m_c=m_\mathcal{Q}$, in particular of the exotic \XYZ states. The kinematics are then given by
%
\begin{subequations}
\begin{align}
 E_a &=  \frac{s-m^2}{2 \sqrt{s}},\quad
 E_b  =  \frac{s+m^2}{2 \sqrt{s}},\quad
 E_c  =  \frac{s+m_\mathcal{Q}^2-M^2}{2 \sqrt{s}} \\
|p_a|&=|p_b| = \frac{\lambda^{1/2}(s,0,m^2)}{2 \sqrt{s}},\quad
 |p_c| = \frac{\lambda^{1/2}(s,m_\mathcal{Q}^2,M^2)}{2 \sqrt{s}},
\end{align}
\end{subequations}
%
where $E_i$ and $|p_i|$ are the particle energies and absolute values of the three-momenta $\bm p_i$, respectively, in the center-of-mass frame.
As usual, $\lambda(a,b,c) = a^2+b^2+c^2-2(a b + b c + c a)$. 
%
The scattering angle $\theta$ of particle $c$ in the center-of-mass system is determined by
%
\begin{equation}
\cos \theta = \frac{s(t-u) - m^2(m_\mathcal{Q}^2-M^2)}{\lambda^{1/2}(s,0,m^2) \lambda^{1/2}(s,m_\mathcal{Q}^2,M^2)},
\end{equation}
noting that the relation $s+t+u=m^2+m_\mathcal{Q}^2+M^2$ holds.
%
It is convenient to introduce the kinematical variable $x$, which fulfills
%
\begin{equation}
    s+t-2E_bE_c-2p_b\frac{\lambda^{1/2}(s,m_\mathcal{Q}^2,m^2)}{2\sqrt{s}}x=M^2.
\end{equation}
%
 The cross sections of semi-inclusive photoproduction are then generally written as
%
\begin{equation}
E_c \frac{\mathrm{d}^3 \sigma}{\mathrm{d}^3 \bm p_c} = \frac{2|p_a| \sqrt{s}}{\pi} \frac{\mathrm{d}^2 \sigma}{\mathrm{d} t \mathrm{d} M^2}=   \frac{1}{\pi} \frac{s-m^2}{\lambda^{1/2}(s,m_\mathcal{Q}^2,M^2)} \frac{\mathrm{d}^2 \sigma}{\mathrm{d} t \mathrm{d} x} .
\end{equation}
%
The exclusive cross section is recovered at the pole
%
\begin{equation}
    \frac{\mathrm{d}\sigma}{\mathrm{d}t}=\pi
\int\mathrm{d}M^2  \frac{\mathrm{d}^2\sigma}{\mathrm{d}t\mathrm{d}M^2}\delta(M^2-m^2).
\end{equation}
\astrid{Should there really be a factor $\pi$?}

From a different perspective, since the 1970's (semi-)inclusive electron scattering off protons has been the main experimental tool to scrutinize the inner structure of nucleons. Data on the corresponding cross sections and structure functions have been key ingredients in global QCD analyses of parton (quark and gluon constituents) distributions~\cite{Collins:1989gx,Harland-Lang:2014zoa, Dulat:2015mca, Ball:2017nwa, Moffat:2021dji, Accardi:2016qay, Sato:2019yez, Alekhin:2017kpj,Abele:2021nyo,Liu:2021jfp}. High-precision measurements of inclusive electron scattering cross sections in the resonance region were made at Jefferson Lab Halls~B and~C~\cite{Osipenko:2003bu, Liang:2004tj, Christy:2007ve,Malace:2009kw, Prok:2014ltt, Tvaskis:2016uxm,Golubenko:2019gxz}.

Being able to describe the strong interaction physics across a broad range of energy and distance scales is crucial, but the non-perturbative regime is still far from being well understood, and in particular the transition from the low-energy resonance region to the high-energy (deep inelastic scattering) regime offers broad grounds for exploration~\cite{ Feynman:1972xm, Farrar:1975yb, Close:1988br, Melnitchouk:1995fc, Brady:2011uy, Owens:2012bv,Nocera:2014uea,Accardi:2016qay, Alekhin:2017kpj, Moffat:2019qll}. Leading twist approximations (leading term in expansions in inverse powers of 
$Q^2$) are found to be accurate at describing the energy region above the invariant mass $W$ of resonance excitations and at sufficiently large photon virtualities, $Q^2 \gtrsim 1-2\gevnospace^2$. Therefore, global QCD analyses~\cite{Accardi:2016qay, Alekhin:2017kpj, Sato:2019yez} usually involve cuts in $W$ and $Q^2$~\cite{,Jimenez-Delgado:2013sma,Harland-Lang:2014zoa, Dulat:2015mca, Ball:2017nwa, Gao:2017yyd, Ethier:2020way, Moffat:2021dji}. In order to bridge the perturbative and nonperturbative regimes and to assess the parton distributions at large $x$, target mass corrections, higher twists and factorization breaking corrections are called for. In addition, due to the resonance peaks appearing in the $W<2\gev$ region, the electroexcitation amplitudes of the resonances should be incorporated into the description of the structure functions~\cite{HillerBlin:2019jgp,Blin:2021twt}.

 A further motivation for these studies is the phenomenologically observed~\cite{Bloom:1970xb} duality between the structure functions in the nucleon resonance region, when averaged over resonances, and the scaling function extrapolated from the deep-inelastic scattering region.
When integrating the structure functions over (finite intervals of) $x$, one obtains the (truncated) moments of the structure functions~\cite{Forte:1998nw, Forte:2000wh}.
The leading twist term is associated with incoherent scattering with individual partons in the nucleon~\cite{Piccione:2001vf, Kotlorz:2006dj, Kotlorz:2016icu}, while the higher twist corrections capture elements of long-distance, nonperturbative quark-gluon dynamics associated with color confinement in QCD~\cite{Ji:1994br,Psaker:2008ju}. Duality is interpreted as the dominance of the leading twist and suppression of higher twist contributions to the moments~\cite{DeRujula:1976baf}.

The inclusive structure functions are related to the total virtual photon--nucleon scattering cross sections $\sigma_T$ and $\sigma_L$, for transversely and longitudinally polarized photons, respectively~\cite{Drechsel:2002ar},
%
\begin{subequations}
\label{sf} 
\begin{align}
F_1(W,Q^2) &=\frac{{K m}}{4\pi^2\alpha}\, \sigma_T(W,Q^2),  \\
F_2(W,Q^2) &=\frac{{K m}}{4\pi^2\alpha}\, \frac{2x}{\rho^2}
             \left(\sigma_T(W,Q^2) +\sigma_L(W,Q^2)\right),
\end{align}
\end{subequations}
%
where $\alpha$ is Sommerfeld's fine structure constant, $K$ is the equivalent photon energy, defined here in the Hand convention as
%
\begin{align}
K&=\frac{W^2-m^2}{2m},
\end{align}
%
and $\rho$ is a kinematic parameter,
%
\begin{align}
\rho^2 = 1 + \frac{4 m^2 x^2}{Q^2}.
\label{rhopar}
\end{align}
%
The $F_2$ structure function can also be written in terms of the unpolarized virtual photoproduction cross section~$\sigma_{U}$,
%
\begin{align}
\label{eq:F2sig}
F_2(W,Q^2)
& = \frac{K m}{4\pi^2\alpha} 
    \frac{2x}{\rho^2} 
    \frac{1+R_{LT}}{1+\epsilon R_{LT}}\, \sigma_{U}(W,Q^2),
\end{align}
%
where
%
\begin{equation}
\label{xs}
\sigma_{U}(W,Q^2) = \sigma_T(W,Q^2) + \epsilon\, \sigma_L(W,Q^2),
\end{equation}
%
and $\epsilon$ is the degree of transverse virtual photon polarization, determined by the scattered electron angle, $\theta_e$, in the laboratory frame and the parameter $\rho$ in Eq.~(\ref{rhopar}),
%
\begin{equation}
\epsilon = \left( 1 + \frac{2 \rho^2}{\rho^2-1} \tan^2\frac{\theta_e}{2}
           \right)^{-1}.
\label{SigmaU1}
\end{equation}
%
In Eq.~(\ref{eq:F2sig}) $R_{LT}$ is the ratio of longitudinal to transverse virtual photon cross sections,
%
\begin{equation}
\label{rlt}
R_{LT}(W,Q^2)=\frac{\sigma_{L}(W,Q^2)}{\sigma_{T}(W,Q^2)}.
\end{equation}
%
The longitudinal structure function is defined as
%
\begin{equation}
F_L(W,Q^2) =\frac{K M}{4\pi^2\alpha} 
    2x\,\sigma_L(W,Q^2)= \rho^2 F_2(W,Q^2) - 2 x F_1(W,Q^2).
\label{sfl}
\end{equation}
